Helping Figures Tell their Story! Paper-Grounded Video Generation Explaining Complex Scientific Figures

Scientific figures compress complex pipelines into a single canvas, yet understanding them requires paper-grounded, step-by-step narration aligned with visual highlights a capability missing from current video generation systems and benchmarks. To address this, we introduce paper-grounded figure-to-video generation: generating narrated, region-grounded walkthrough videos from a figure and its paper. We propose MINARD (Multimodal Interpretation of Narrated Architecture via Region Decomposition), a pipeline that generates paper-grounded narrations and sequentially grounds them to figure regions. We also release FigTalk, a benchmark with new sequential and component-level grounding metrics derived. On FigTalk, MINARD generates humanlike, paper-faithful narrations and outperforms narration-conditioned figure spatial grounding compared to existing approaches in both automatic and human evaluation

==> acl_lualatex.tex <==
% % This file compiles with both LuaLaTeX and XeLaTeX
% \documentclass[11pt]{article}

% % Change "review" to "final" to generate the final (sometimes called camera-ready) version.
% % Change to "preprint" to generate a non-anonymous version with page numbers.
% \usepackage[review]{acl}

% % This is not strictly necessary, and may be commented out,
% % but it will improve the layout of the manuscript,
% % and will typically save some space.
%  \usepackage{microtype}

% % If the title and author information does not fit in the area allocated, uncomment the following
% %
% %\setlength\titlebox{<dim>}
% %
% % and set <dim> to something 5cm or larger.

% % These font selection commands work with
% % LuaLaTeX and XeLaTeX, but not pdfLaTeX.
% \usepackage[english,bidi=default]{babel} % English as the main language.
% \babelfont{rm}{TeXGyreTermesX} % similar to Times
% %%% include whatever languages you need below this line
% \babelprovide[import]{hindi}
% \babelfont[*devanagari]{rm}{Lohit Devanagari}
% \babelprovide[import]{arabic}
% \babelfont[*arabic]{rm}{Noto Sans Arabic}


% %\usepackage{polyglossia}
% %\setdefaultlanguage{english}
% %\setotherlanguages{arabic,russian,thai,hindi,kannada}

% %%%%%


% \title{LuaLaTeX and XeLaTeX Template for *ACL Style Files}

% % Author information can be set in various styles:
% % For several authors from the same institution:
% % \author{Author 1 \and ... \and Author n \\
% %         Address line \\ ... \\ Address line}
% % if the names do not fit well on one line use
% %         Author 1 \\ {\bf Author 2} \\ ... \\ {\bf Author n} \\
% % For authors from different institutions:
% % \author{Author 1 \\ Address line \\  ... \\ Address line
% %         \And  ... \And
% %         Author n \\ Address line \\ ... \\ Address line}
% % To start a seperate ``row'' of authors use \AND, as in
% % \author{Author 1 \\ Address line \\  ... \\ Address line
% %         \AND
% %         Author 2 \\ Address line \\ ... \\ Address line \And
% %         Author 3 \\ Address line \\ ... \\ Address line}

% \author{First Author \\
%   Affiliation / Address line 1 \\
%   Affiliation / Address line 2 \\
%   Affiliation / Address line 3 \\
%   \texttt{email@domain} \\\And
%   Second Author \\
%   Affiliation / Address line 1 \\
%   Affiliation / Address line 2 \\
%   Affiliation / Address line 3 \\
%   \texttt{email@domain} \\}

% \begin{document}

% \maketitle
% \begin{abstract}
% This document provides an example showing how
% to use the *ACL style files with either
% LuaLaTeX or XeLaTeX.
% \end{abstract}


% \section{Introduction}

% Please see the general instructions
% in the file \verb|acl_latex.tex|.

% Here are some examples of text in various languages.

% Hindi: \foreignlanguage{hindi}{मानव अधिकारों की सार्वभौम घोषणा}

% Arabic: \foreignlanguage{arabic}{الإعلان العالمي لحقوق الإنسان}

% Here is an example citation:
% \citet{Gusfield:97} argues that...


% % Entries for the entire Anthology, followed by custom entries
% \bibliography{custom}

% \appendix

% \section{Example Appendix}
% \label{sec:appendix}

% This is an appendix.

% \end{document}

